The s-Process in Low Metallicity Stars. II. Interpretation of High-Resolution Spectroscopic Observations with AGB models

High-resolution spectroscopic observations of a hundred metal-poor Carbon and s-rich stars (CEMP-s) collected from the literature are compared with the theoretical nucleosynthesis models of asymptotic giant branch (AGB) presented in Paper I (M = 1.3, 1.4, 1.5, 2 Msun, -3.6 < [Fe/H] < -1.5). The s-process enhancement detected in these objects is associated to binary systems: the more massive companion evolved faster through the thermally pulsing AGB phase (TP-AGB), synthesising in the inner He-intershell the s-elements, which are partly dredged-up to the surface during the third dredge-up (TDU) episode. The secondary observed low mass companion became CEMP-s by mass transfer of C and s-rich material from the primary AGB. We analyse the light elements as C, N, O, Na and Mg, as well as the two s-process indicators, [hs/ls] (where ls = <Y, Zr> is the the light-s peak at N = 50 and hs = <La, Nd, Sm> the heavy-s peak at N = 82), and [Pb/hs]. We distinguish between CEMP-s with high s-process enhancement, [hs/Fe] > 1.5 (CEMP-sII), and mild s-process enhanced stars, [hs/Fe] < 1.5 (CEMP-sI). To interpret the observations, .... . Detailed analyses for individual stars will be provided in Paper III.

==> tableA1_revised2.tex <==
 
\begin{table}
\captionsetup[wraptable]{name=Table A1.}  
\caption*{\label{tablebinary} {\bf Table A1.} Binarity status of the star sample.
For the stars not listed here there are no measurements available so far.
The label ``no confirmation'' means that the velocity amplitude is
 too low to confirm binary motion, while ``p. v. v.?'' indicates 
 stars with too short observation time (see Section~2).
 References are the same as in Table~1, as well 
as Aoki et al. (2000, 2003), A00, A03, Lucatello et al. (2009), L09, Lucatello et al. (2005), L05,
Jorissen et al. (2005), Jor05, McClure \& Woodsworth (1990), MC90, Norris et al. (1997), N97, 
Preston (2009), P09, Preston \& Sneden (2000), PS00, Sivarani et al. (2004), S04.}
\begin{center} 
%\begin{minipage}{\textwidth}                         
\begin{tabular}{lll}                 
\hline
Stars & Binary (period in days) & Ref.\\
\hline
BD+04$^{\circ}$2466 & yes (P = 4592.7 $\pm$ 51.1 d) & Jor05 \\
BS 16080$-$175 &   p. v. v.? & T05 \\	
BS 17436$-$058 &  no & T05 \\
CS 22183$-$015   &     p. v. v.? & T05  \\%***QUI\\tolto si da Cohen et al. (\cite{cohen06}), Lai et al. (\cite{lai04})
CS 22880$-$074    &     no & PS01, A02c, T05, P09     \\     
CS 22881$-$036    &       no, yes (P = 378 d) & PS01, A02c, P09     \\  
CS 22887$-$048 &    yes & T05 \\
CS 22898$-$027    &   no &  PS01, A02c, T05, P09		    \\
CS 22942$-$019    & yes (P = 2800 d; 3616 d)& PS01; L09        \\
CS 22948$-$27     & yes (P = 426.5 d; 425.1 d)& PS01, BB05, A08; L09      \\
CS 22956$-$028   &   yes (P = 1290 d; 1312 d) & S03; L09 \\
CS 22964$-$161    & 	yes (triple?), P = 252 d	&	T08\\	
CS 29497$-$030    &     yes (P = 342 d) & PS00, S04, S03  \\
CS 29497$-$34     &      yes (P = 4130 d; 471 d) & PS01, BB05, A08; L09		\\
CS 29509$-$027   &   yes (P = 194 d) & S03 \\
CS 29503$-$010    &   	no & T05						          \\              
CS 29526$-$110    & yes & A02d, A08, T05	\\	
CS 29528$-$028    & 	no & T05			          \\          
CS 30301$-$015    &  p. v. v.? & T05  \\   
CS 30322$-$023    & no confirmation & M06\\
CS 31062$-$012   &   no; yes (P = 1130 d) & N97, A08; L09\\
CS 31062$-$050    &  yes & A03, T05	      \\ 
%HD 187216 & cercare ***QUI & \citet{kipper94} \\    
HD 5223         & yes; 755.2 d & MC90 \\
HD 196944       &    yes & T05, L05   	\\
HD 198269       & yes; 1295 d & MC90\\
HD 201626       & yes; 1465 d & MC90\\
HD 209621       & yes; 407.4 d &MC90\\
HE 0012$-$1441  &        yes	&	C06 \\				
HE 0024$-$2523  & yes (P = 3.41 d)   &    L03     \\  
HE 0338$-$3945  & 	no & J06			\\		
HE 2148$-$1247  & yes (P $\geq$ 4400 d\footnote{long period with small amplitude.})  &   C03 \\			                                            
LP 625$-$44     & yes (P = 4547 d) & L09, N97, A00, T05\\
HK-II 17435$-$00532	&		no confirmation & R08	\\
SDSS 1707+58 & yes (P short, triple?) & A08 \\ 	
\hline  
\end{tabular}  
%\end{minipage} 
\end{center}     
\end{table} 


==> tableA2_revised2.tex <==
\begin{table}
\captionsetup[wraptable]{name=Table A2.}
\caption*{\label{abbsolar} {\bf Table A2.} Solar meteoritic abundance determinations by Anders \& Grevesse (1989), (AG89$_{\rm m}$)
compared with solar photospheric abundance determinations by Lodders et al. (2009), (L09$_{\rm ph}$).
Only heavy elements with differences higher than 0.05 dex are listed here
(Sr, Y and Zr show negligile differences, $\leq$ 0.03).
The difference between the two iron values is $\Delta$(log $\epsilon$(Fe)) =  7.51 - 7.45 = 0.06.}
\begin{center}
\begin{tabular}{l|ccc}
\hline 
Element  &AG89$_{\rm m}$&  L09$_{\rm ph}$ &    AG89$_{\rm m}$ $-$ L09$_{\rm ph}$  \\
\hline             
%%%He   2   &  10.99   &    10.925   &        0.06   \\        
%%%C    6   &  8.56*    &    8.39     &        0.17   \\        
%%%N    7   &  8.05*    &    7.86     &        0.19   \\        
%%%O    8   &  8.93*    &    8.73     &        0.20   \\        
%%F    9   &  4.48    &     4.56    &         -0.08 \\        
%%%Ne   10  &  8.09    &     8.05    &         0.04  \\        
%%%Na   11  &  6.31    &    6.30      &       0.01    \\        
%%%Mg   12  &  7.58    &    7.54     &        0.04   \\        
%%%Al   13  &  6.48    &    6.47     &        0.01   \\        
%%%Si   14  &  7.55    &    7.52     &        0.03   \\        
%%P    15  &  5.57    &     5.46    &         0.11  \\        
%%S    16  &  7.27    &     7.14    &         0.13  \\        
%%Cl   17  &  5.27    &     5.50     &        -0.23  \\        
%%Ar   18  &  6.56    &    6.50      &       0.06    \\        
%%%K    19  &  5.13    &    5.12     &        0.01   \\        
%%%Ca   20  &  6.34    &    6.33     &        0.01   \\        
%%%Sc   21  &  3.09    &     3.10     &        -0.01  \\        
%%%Ti   22  &  4.93    &     4.90     &        0.03   \\        
%%%V    23  &  4.02    &    4.00        &     0.02      \\        
%%%Cr   24  &  5.68    &    5.64     &        0.04   \\        
%%Mn   25  &  5.53    &     5.37    &         0.16  \\        
%%Fe   26  &  7.51    &     7.45    &         0.06  \\        
%%%Co   27  &  4.91    &    4.92     &        -0.01  \\        
%%%Ni   28  &  6.25    &    6.23     &        0.02   \\        
%%Cu   29  &  4.27    &     4.21    &         0.06  \\        
%%%Zn   30  &  4.65    &    4.62     &        0.03   \\        
%%Ga   31  &  3.13    &     2.88    &         0.25  \\        
%%Ge   32  &  3.63    &     3.58    &         0.05  \\        
%%As   33  &  2.37    &     2.32    &         0.05  \\        
%%%Se   34  &  3.35    &    3.36     &        -0.01  \\        
%%Br   35  &  2.63    &    2.56     &        0.07   \\        
%%Kr   36  &  3.23    &     3.28    &         -0.05 \\        
%%Rb   37  &  2.40    &     2.60     &        -0.20  \\        
%Sr   38  &  2.93    &    2.92     &        0.01   \\        
%Y    39  &  2.22    &    2.21     &        0.01   \\        
%Zr   40  &  2.61    &    2.58     &        0.03   \\        
%Nb   41  &  1.40    &    1.42     &        -0.02  \\        
%Mo   42  &  1.96    &    1.92     &        0.04   \\         
                                                 
%%%Ru   44  &  1.82    &    1.84     &        -0.02  \\        
%%%Rh   45  &  1.09    &    1.12     &        -0.03  \\        
%%%Pd   46  &  1.70    &    1.66     &        0.04   \\        
%%Ag   47  &  1.24    &    0.94     &        0.30   \\        
%%%Cd   48  &  1.76    &    1.77     &        -0.01  \\        
%%%In   49  &  0.82    &    0.78     &        0.04   \\        
%%Sn   50  &  2.14    &     2.00     &        0.14   \\        
%%%Sb   51  &  1.04    &    1.00      &       0.04    \\        
%%%Te   52  &  2.24    &    2.20      &       0.04    \\        
%%I    53  &  1.51    &    1.57     &        -0.06  \\        
%%%Xe   54  &  2.23    &    2.27     &        -0.04  \\        
%%%Cs   55  &  1.12    &    1.10      &       0.02    \\        
%Ba   56  &  2.21    &    2.17     &        0.04   \\        
La    &  1.20    &     1.14    &         0.06  \\        
%Ce   58  &  1.61    &    1.61     &        0.00   \\        
%Pr   59  &  0.78    &     0.76    &         0.02  \\        
%Nd   60  &  1.47    &    1.45     &        0.02   \\        
                                                 
%Sm   62  &  0.97    &    1.00     &        -0.03  \\        
%Eu   63  &  0.54    &    0.52     &        0.02   \\        
Gd     &  1.07    &     1.11    &         $-$0.04 \\        
Tb     &  0.33    &     0.28    &         0.05  \\        
%Dy   66  &  1.15    &    1.13     &        0.02   \\        
%Ho   67  &  0.50    &    0.51     &        -0.01  \\        
%Er   68  &  0.95    &    0.96     &        -0.01  \\        
%Tm   69  &  0.13    &    0.14     &        -0.01  \\        
Yb     &  0.95    &     0.86    &         0.09  \\        
%Lu   71  &  0.12    &     0.12    &         0.00  \\        
Hf     &  0.73    &     0.88    &         $-$0.15 \\        
%Ta   73  &  -0.13   &    -0.14    &        0.01   \\        
W      &  0.68    &    1.11     &        $-$0.43  \\        
%Re   75  &  0.27    &    0.28     &        -0.01  \\        
Os     &  1.38    &     1.45    &         $-$0.07 \\        
%Ir   77  &  1.37    &    1.38     &        -0.01  \\        
Pt    &  1.68    &     1.74    &         $-$0.06 \\        
Au    &  0.83    &    1.01     &        $-$0.18  \\        
Hg    &  1.09    &     1.19    &         $-$0.10 \\        
Tl    &  0.82    &    0.95     &        $-$0.13  \\        
Pb    &  2.05    &     2.00     &        0.05   \\        
%Bi   83  &  0.71    &    0.67     &        0.04   \\            
\hline                                                     
\end{tabular}
\end{center}  
\end{table}                                                           
                                                        
                                                            
                                                            
